First Provably Optimal Asynchronous SGD for Homogeneous and Heterogeneous Data

Artificial intelligence has advanced rapidly through large neural networks trained on massive datasets using thousands of GPUs or TPUs. Such training can occupy entire data centers for weeks and requires enormous computational and energy resources. Yet the optimization algorithms behind these runs have not kept pace. Most large scale training still relies on synchronous methods, where workers must wait for the slowest device, wasting compute and amplifying the effects of hardware and network variability. Removing synchronization seems like a simple fix, but asynchrony introduces staleness, meaning updates computed on outdated models. This makes analysis difficult, especially when delays arise from system level randomness rather than algorithmic choices. As a result, the time complexity of asynchronous methods remains poorly understood. This dissertation develops a rigorous framework for asynchronous first order stochastic optimization, focusing on the core challenge of heterogeneous worker speeds. Within this framework, we show that with proper design, asynchronous SGD can achieve optimal time complexity, matching guarantees previously known only for synchronous methods. Our first contribution, Ringmaster ASGD, attains optimal time complexity in the homogeneous data setting by selectively discarding stale updates. The second, Ringleader ASGD, extends optimality to heterogeneous data, common in federated learning, using a structured gradient table mechanism. Finally, ATA improves resource efficiency by learning worker compute time distributions and allocating tasks adaptively, achieving near optimal wall clock time with less computation. Together, these results establish asynchronous optimization as a theoretically sound and practically efficient foundation for distributed learning, showing that coordination without synchronization can be both feasible and optimal.

==> Nomenclature.tex <==
%\chapter*{Nomenclature}
%\ \vfill \centerline{\Huge \bf NOMENCLATURE} \vfill \ 

%\addcontentsline{toc}{chapter}{Nomenclature}
%\cleardoublepage

\chapter*{\center\Huge{ACRONYMS}}


\addcontentsline{toc}{chapter}{Acronyms}
%\addcontentsline{lot}{chapter}{Acronyms}

%\begin{table}[h!]
%\begin{center}
%\caption{Acronyms}
%\resizebox{1\textwidth}{!}
%{
%\renewcommand{\baselinestretch}{1.3}
\begin{center}
\small
\begin{longtable}{ll}\hline  
\textbf{Symbol} & \textbf{Meaning}\\\hline
CA & Cellulose Acetate\\
CE & Cellulose Ester\\
COC & Cyclic Olefin Copolymer\\
CTE &Coefficient of Thermal Expansion\\
EMPIRe & Electromechanical Microsystems and Polymer Integration Research\\
EOF & Electro-Osmotic Flow\\
HAA & Heat Activated Adhesive\\


\hline
\end{longtable} 
\end{center}
%\renewcommand{\baselinestretch}{1.75}

\chapter*{\center\Huge{LIST OF SYMBOLS}}


\addcontentsline{toc}{chapter}{List of Symbols}
%\addcontentsline{lot}{chapter}{List of Symbols}

%\renewcommand{\baselinestretch}{1.3}
\begin{center}
\begin{tabular}{ll}\hline
\textbf{Symbol} & \textbf{Meaning}\\\hline
CO$_2$ & Carbon dioxide\\
KOH& Potassium Hydroxide\\ 
$P$ & Laser power\\
$P_b$ & Bonding pressure\\
$s$ & Laser speed\\
$t_b$ & Bonding time\\
$t_c$ & Cooling time\\
$t_{comp}$ & Compression time\\
$t_h$ & Heating time\\

\hline
\end{tabular}
\end{center}
%\renewcommand{\baselinestretch}{1.75}


==> Papers.tex <==

% Appendix for Papers

\refstepcounter{chapter}%
\chapter*{\thechapter \quad Papers Submitted and Under Preparation (In Order of Preparation)}

\paragraph{Papers Before PhD}
\begin{enumerate}
    \item martin
    \item Gradskip?
\end{enumerate}    

\paragraph{Papers During PhD}
\begin{enumerate}
    \item Gradskip?
    \item \bibentry{condat2025locodl}
    \item \bibentry{maranjyan2025mindflayer}
    \item \bibentry{maranjyan2024differentially}
    \item \bibentry{maranjyan2025ringmaster}
    \item \bibentry{maranjyan2025ata}
    \item \bibentry{maranjyan2025ringleader}
\end{enumerate}

% $\bullet$ Author 1 Name, Author 2 Name, and Author 3 Name, {``Article Title"}, \emph{Submitted to Conference/Journal Name}, further attributes.\\
% $\bullet$ Author 1 Name, Author 2 Name, and Author 3 Name, {``Article Title"}, \emph{Submitted to Conference/Journal Name}, Mon. Year. \\
% $\bullet$ Author 1 Name, Author 2 Name, and Author 3 Name, {``Article Title"}, \emph{Submitted to Conference/Journal Name}, Mon. Year.

